Analysis of thermochemical non-equilibrium hypersonic flow over a waverider with uncertainty quantification

The objective of this work is to assess the impact of parameter uncertainty on hypersonic aerothermal surface heating predictions in Reynolds-Averaged Navier-Stokes (RANS) simulations using non-intrusive uncertainty quantification (UQ) techniques. RANS-based models are considered indispensable tools in computational fluid dynamics (CFD) analysis for the iterative and cost-effective exploration of innovative design concepts. However, these RANS models heavily rely on empirical constants that often require tuning due to the lack of physical knowledge and complexity of the problem, introducing significant uncertainties that hinder their predictive capabilities. Therefore, this research investigates the influence of the turbulent Prandtl number uncertainty, that governs the level of shear stress and heat flux present in the turbulent flow, on key output quantities of interest (QoIs). The US3D hypersonics solver is employed to simulate aeroheating over a hypersonic waverider configuration using the classical Menter Shear Stress Transport (SST) turbulence model. A polynomial chaos expansion (PEC) framework is presented that enables a global sensitivity analysis and forward propagation of uncertainty for a range of turbulent prandtl number, generating statistics including skewness and kurtosis of the QoIs. In addition, Sobol indices are calculated to quantify the relative contribution of the turbulent prandtl number to the overall uncertainty in the heat flux and surface pressure outputs. The results provide valuable insights into the underlying aeroheating behavior in RANS simulations under hypersonic non-equilibrium flow conditions over a waverider previously studied at the Arnold Engineering Development Center (AEDC) facility. These findings will inform future design processes and improve the reliability of RANS-based predictions in hypersonic applications.

==> 01abstract.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Abstract:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%The objective of this work is to assess the impact of parameter uncertainty on hypersonic aerothermal surface heating predictions in Reynolds-Averaged Navier-Stokes (RANS) simulations using non-intrusive uncertainty quantification (UQ) techniques. RANS-based models are considered indispensable tools in computational fluid dynamics (CFD) analysis for the iterative and cost-effective exploration of innovative design concepts. However, these RANS models heavily rely on empirical constants that often require tuning due to the lack of physical knowledge and complexity of the problem, introducing significant uncertainties that hinder their predictive capabilities. Therefore, this research investigates the influence of Reynolds Stress turbulence closure model uncertainties on output quantities of interest (QoIs). Using the US3D hypersonic flow solver and a vehicle-scale waverider configuration, the classical Spalart-Almaras and Menter-SST turbulence models are utilized to assess the uncertainty and sensitivity analysis of aeroheating and transition. A polynomial chaos expansion framework is employed; which enables global sensitivity analysis and forward propagation of uncertainty, generating histograms, probability density functions, and Pearson correlation coefficients for the QoIs. In addition, Sobol indices are calculated to quantify the relative contribution of each input uncertainty to the overall uncertainty in the output. The results will provide valuable insights into the underlying aeroheating behavior in RANS simulations under hypersonic non-equilibrium flow conditions over a waverider previously studied at the Arnold Engineering Development Center (AEDC) facility. These findings will inform future design processes and improve the reliability of RANS-based predictions in hypersonic applications.

The objective of this work is to assess the impact of parameter uncertainty on hypersonic aerothermal surface heating predictions in Reynolds-Averaged Navier-Stokes (RANS) simulations using non-intrusive uncertainty quantification (UQ) techniques. RANS-based models are considered indispensable tools in computational fluid dynamics (CFD) analysis for the iterative and cost-effective exploration of innovative design concepts. However, these RANS models heavily rely on empirical constants that often require tuning due to the lack of physical knowledge and complexity of the problem, introducing significant uncertainties that hinder their predictive capabilities. Therefore, this research investigates the influence of the turbulent Prandtl number ($P_{tr}$) uncertainty, that governs the level of shear stress and heat flux present in the  turbulent flow, on key output quantities of interest (QoIs). The US3D hypersonics solver is employed to simulate  aeroheating over a hypersonic waverider configuration using the classical Menter Shear Stress Transport (SST) turbulence model. 
A preliminary study was conducted to demonstrate US3D’s ability to predict the aerodynamic and heat flux parameters with acceptable comparison to experiments for a range of flight conditions. Then, a polynomial chaos expansion (PEC) framework is presented that enables a global sensitivity analysis and forward propagation of uncertainty for a range of $P_{tr}$, generating statistics including skewness and kurtosis of the QoIs. In addition, Sobol indices are calculated to quantify the relative contribution of the $P_{tr}$ to the overall uncertainty in the heat flux and surface pressure outputs. The results provide valuable insights into the underlying aeroheating behavior in RANS simulations under hypersonic non-equilibrium flow conditions over a waverider previously studied at the Arnold Engineering Development Center (AEDC) facility. These findings will inform future design processes and improve the reliability of RANS-based predictions in hypersonic applications.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
